Causal Inference for Time series Analysis: Problems, Methods and Evaluation

Time series data is a collection of chronological observations which is generated by several domains such as medical and financial fields. Over the years, different tasks such as classification, forecasting, and clustering have been proposed to analyze this type of data. Time series data has been also used to study the effect of interventions over time. Moreover, in many fields of science, learning the causal structure of dynamic systems and time series data is considered an interesting task which plays an important role in scientific discoveries. Estimating the effect of an intervention and identifying the causal relations from the data can be performed via causal inference. Existing surveys on time series discuss traditional tasks such as classification and forecasting or explain the details of the approaches proposed to solve a specific task. In this paper, we focus on two causal inference tasks, i.e., treatment effect estimation and causal discovery for time series data, and provide a comprehensive review of the approaches in each task. Furthermore, we curate a list of commonly used evaluation metrics and datasets for each task and provide in-depth insight. These metrics and datasets can serve as benchmarks for research in the field.

==> Evaluation/datasets.tex <==

\subsection{Datasets}
\raha{we need to briefly discuss traditional time series as well}
%\qianru{Raha, I re-wrote this part based on my understanding. If there are some mistakes, please modify it.}

In this section, we briefly introduce some of the datasets used in causal inference literature on time series. 
% In addition, we categorize the datasets based on their properties\raha{please explain what you mean by properties}. Traditional time series data may not have causal ground truth information, thus, in many cases, synthetic datasets are created. 
\qianru{We firstly introduce the traditional time series datasets. Because causality for time series is a extensive problem from traditional problem. To deal with causal treatment estimation and causal discovery, traditional time series datasets still have some limitations that they may not have causal ground truth information. Therefore, we then introduce causal time series datasets including real datasets and  synthetic datasets, which are used to solve causal time series problems.}


% \qianru{The intention of introducing time series data is not clear. Why we need to introduce it?}

\subsubsection{Time Series Datasets}
\mk{As for the traditional datasets, you talked about the UCR dataset in details while the other ones include only a brief description.}

Traditionally time-series analysis has used a variety of data. In one of the more comprehensive surveys on time series models, Fawaz et al.\cite{fawaz2019deep} use 97 time series datasets to evaluate 8,730 deep learning models. The datasets in this study are taken from two time series dataset archives. One of the archives is the UCR Time Series Classification Archive \cite{UCRArchive2018} while the second archive is the one associated with Multivariate Time Series Classification with Learned Discretization \cite{Baydogan}. 

The UCR time series dataset that is used in various other publications \cite{bagnall2015,xing2010brief}, consists of more than 120 datasets. The authors intend that instead of cherry-picking datasets to make claims about a time series approach, researchers should use all the datasets in the archive to ensure the robustness of their approach\cite{UCRArchive2018}. These datasets represent a classification problem. Thus, there is a class label for each item in every dataset in the archive. The length of the time series for each class in a single dataset is the same. Additionally, the classes are independent i.e. something that needs to be classified cannot occur in multiple classes in the ground truth.\remove{The authors provide three benchmarks: Euclidean Distance, Unconstrained DTW, and Constrained DTW with learned warping width.}

Another useful archive containing multivariate time series is Baydogan's archive\cite{baydogan2015learning}. This archive consists of over a dozen diverse multivariate time series datasets.

There are many other time series datasets in use apart from the ones included in the UCR archive. For example, Real/Synthetic Yahoo Network traffic, Synthetic Yahoo Services with Seasonality, Synthetic Yahoo Services with Changepoint Anomalies, and NYC Taxi Dataset are recommended by Braei et al. \cite{braei2020}.

Time series datasets are very useful for various purposes but since this survey is based on Causal Time Series specifically, we look at datasets used in causal literature. We divide these datasets into two categories: Real datasets and Synthetic datasets. 



% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
\begin{table*}[]
	\centering
	\begin{tabular}{|l|p{0.2\textwidth} | p{0.3\textwidth} |p{0.3\textwidth} |}
		\hline
		{} &  \textbf{Model}       & \textbf{Description}                                        & \textbf{Datasets}                                                                                                         \\ \hline
		1 & Autocorelation          & Dependence on time-lagged component                         & 3D-Tensor\cite{schaechtle2013multi}, Complex time-series \cite{runge1702detecting}                                       \\ \hline
		2 & Autoregression          & Dependence on sum of time-lagged components                 & Gong et al., 2015 \cite{gong2017causal}, Bica et al. \cite{bica2019time}, Brodersen et al.\cite{brodersen2015inferring} \\ \hline
		3 & Confounding             & Multiple effects from the same cause                        & Bica et al. \cite{bica2019time}                                                                                          \\ \hline
		4 & Non-linear           & Absence of a linear relationship between cause and effect   & Financial Time-Series \cite{kleinberg2013causal}, Particle Simulation \cite{lowe2020amortized}                            \\ \hline
		5 & Dynamic Time dependence & Dependence on the time-lagged component(s) varies over time & Li et al. \cite{li2018estimating}                                                                                        \\ \hline
		6 & Chaotic              & Small changes in parameters create large changes over time  & Papana et al. \cite{papana2013simulation}, Khanna et al. \cite{khanna2019economy}                                       \\ \hline
	\end{tabular}
    
\caption{Properties of synthetic datasets used in literature \raha{for which task??}}
\label{tbl:synthetic}
\end{table*}


\begin{comment}
	content...

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table*}[]
	\begin{tabular}{@{}l p{0.1\textwidth} l p{0.3\textwidth} l p{0.3\textwidth} l@{}}
		\toprule
		& Property                & Description                                                 & Datasets                                                                                                                  \\ \midrule
		1 & Autocorelation          & Dependence on time-lagged component                         & 3D-Tensor \cite{schaechtle2013multi}, Complex time-series \cite{runge1702detecting}                                       \\
		2 & Autoregression          & Dependence on sum of time-lagged components                 & Gong et al., 2015 \cite{gong2017causal}, Bica et al. \cite{bica2019time}, Brodersen et al.\cite{brodersen2015inferring} \\
		3 & Confounding             & Multiple effects from the same cause                        & Bica et al. \cite{bica2019time}                                                                                          \\
		4 & Non-linearity           & Absence of a linear relationship between cause and effect   & Financial Time-Series \cite{kleinberg2013causal}, Particle Simulation \cite{lowe2020amortized}                            \\
		5 & Dynamic Time dependance & Dependance on the time-lagged component(s) varies over time & Li et al. \cite{li2018estimating}                                                                                        \\
		6 & Chaoticity              & Small changes in parameters create large changes over time  & Papana et al. \cite{papana2013simulation}, Khanna et al. \cite{khanna2019economy}                                       \\ \bottomrule
	\end{tabular}
\end{table*}
\end{comment}

\qianru{ Please give a table to introduce the datasets for causal estimation and causal discovery problems. You can use the following template as a reference and select some typical dataset to fill in the table.}
\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c}
        Problem & Features in dataset (Description) & Dataset\\ \hline
        \multirow{2}{*}{Causal estimation} & \multirow{2}{*}{treatments, groudtruth,xxx }& real datasets: \\ \cline{3-3}
        & & synthetic datasets:\\\hline
    \end{tabular}
    \caption{Caption}
    \label{tab:my_label}
\end{table*}

\subsubsection{Real Datasets for Causal Time Series}
% \raha{you should have two subsections one for causal effect estimation and one for causal discovery}
\mk{There are no connection between the listed datasets. At least it would have been better if you categorize them somehow.}

Real Datasets used in causal inference for time-series can vary from economic data \cite{gong2017causal} to health data \cite{schaechtle2013multi}. It is ideal to collect the Causal data from randomized experiments. However, in many cases, randomized experiments are unfeasible, as discussed in Section \ref{sec:causal_background}. Therefore, in many cases, we see observational data being used in the literature. 
% \qianru{Maybe we can introduce the datasets here according to the categories of causal inference. You already introduce the datasets well, they will seem structural if organize them using some categories.  Please refer to the following example to re-organize this part. 
% i.e., For causal discovery problem, the dataset should contain xxxxx(some elements, such as what groundtruth looks like). Then tell some datasets as examples.
% For causal treatment estimation, besides elements in causal discovery, the datasets need some treatments or xxxxxx. And the groundtruth is different from causal discovery. Then tell some datasets as examples. In xxx dataset, the author take xxx as treatments, and xxxx as groundtruth.}

One of the examples of real data used for Causal Discovery for Time Series is the US manufacturing growth data used by Entner et al. \cite{entner2010causal}. Growth  rates  of  US  manufacturing firms  in  terms  of  employment,  sales,  research and development expenditure, and operating income are included in this dataset. 
% \raha{please explain about the data, what is the groundtruth and how it is collected, in this section we do not focus on authors findings} %The authors claim to have found a link between employment and sales growth.
\qianru{We classify the causal time series datasets according to the categories of causal problems.}
% \qianru{Maybe we can introduce the datasets here according to the categories of causal inference. You already introduce the datasets well, they will seem structural if organize them using some categories.  Please refer to the following example to re-organize this part. 
% i.e., For causal discovery problem, the dataset should contain xxxxx(some elements, such as what groundtruth looks like). Then tell some datasets as examples.
% For causal treatment estimation, besides elements in causal discovery, the datasets need some treatments or xxxxxx. And the groundtruth is different from causal discovery. Then tell some datasets as examples. In xxx dataset, the author take xxx as treatments, and xxxx as groundtruth.}

\qianru{Please try to summary the datasets. If some datasets have similar feature, you should introduce the features in a abstract way first, such as time-invariant/varying intervention, single/multiple intervention. Then give some examples, who use xxxx. 
Please put the similar datasets together.
}

\qianru{\textbf{Datasets for casual effect:}}
\qianru{*************Please introduce some basic features of datasets for causal effect here*********** }
Health-related datasets are used for causal inference. Schaechtle et al.~\cite{schaechtle2013multi} use a Diabetes dataset by Frank and Asuncion where the ground truth is available. This dataset contains the Glucose curves and insulin dose for 69 patients.

Schaechtle et al.~\cite{schaechtle2013multi} also used Two Variable dataset with Cause-Effect pairs~\cite{mooij2016distinguishing}. It is a growing dataset with diverse data. Thus, it is suitable for benchmarking causal detection algorithms.  Gong et al.~\cite{gong2017causal} use this dataset for causal discovery as well as the Macroeconomic Real Dataset which contains the cause-effect variables real balance and price inflation.
% \raha{please explain how, you can find it in their experiment section}

Another common real dataset is the MIMIC II/III \cite{johnson2016mimic}. This dataset consists of data about patients in ICU. Various attributes about the patients are stored in this database. Examples include blood pressure, oxygen saturation, given medicine, as well as temporal attributes. Thus, it is a goldmine for causal research. This dataset has been used by Bica et al.~\cite{bica2019time} to estimate treatment effects. The dialysis subset of this data has been used by Soleimani et al. for Treatment-Response modeling using counterfactual reasoning~\cite{soleimani2017treatment}.
Brodersen et al.~\cite{brodersen2015inferring} use advertisement data by Google to determine the causal impact. An advertisement campaign was analyzed by the authors where the product ads were placed alongside search results for a period time of 6 weeks. The ad data was used as an intervention to measure the impact on sale volume as the effect.




Li et al.~\cite{li2018estimating} use geo experiment data as one of the experiments for their approach. They use the public geo experiment data provided by Kerman et al.~\cite{kerman2017estimating}. This data consists of an ad campaign as a treatment for half of the nonoverlapping geo data in the sample. 

In a case study about the economic cost of conflict Abadie et al.~\cite{abadie2003economic} use economic data for Spanish regions to analyze the effects of terrorism. The authors use the per capita GDP of Basque over time to do their causal analysis. The data does not have a ground truth value.

Another work by Abadie et al. looks at the effects of California's tobacco control program in their work using Synthetic Control Methods~\cite{abadie2010synthetic}. Here they use annual state-level panel data. This data contains the per-capita cigarette sales from 1970-2000 for multiple US states. This is the time between which Proposition 99 was passed. 

Hausman et al. use air quality data from Auffhammer and Kellogg~\cite{auffhammer2011clearing} over time. Originally, this dataset was used to study the effects of gasoline content on air quality. This dataset includes Ozone levels, minimum/maximum/mean temperatures, precipitation, and snow information. The data goes over the years 1989 till 2006. 

Pfister et al.~\cite{pfister2019invariant} use monetary policy data from three different sources. Quarterly GDP for Switzerland and Euro are taken from Eurostat. The monthly business confidence index and monthly consumer price index for Switzerland are taken from OECD. Monthly balance sheet data, monthly call money rate, and monthly average exchange rate are taken from the Swiss National Bank. By combining all of these data sources, the authors satisfy their goal of finding monthly causal predictors for log-returns of the Euro-Swiss franc exchange rate. The authors use data from the year 1999 to 2017.


A dataset by the Office of Hydrologic Development at the National Oceanic and Atmospheric Administration (OHD-NOAA) is used for Causal Discovery by Jangyodsuk et al.~\cite{jangyodsuk2014causal}. This dataset contains 32 hydrology related variables over several square areas for the entirety of the US except for Alaska and Hawaii. The data is collected at constant intervals of 6 hours and ranged from the years 1979 to 2008. The dataset contains variables like snow depth, subsurface flow component, liquid water storage, and evapotranspiration.

Real-time Whole-brain imaging was used to record the neural activity of Caenorhabditis elegans for creating a dataset used for Causal Discovery by Davis et al.~\cite{davis2006relationship}. The organism has 302 neurons. The dataset is used to which neurons are responsible for movement. The movements of worms in conjunction with neural activity can be used for cause and effect.

\qianru{\textbf{Datasets for causal discovery:}}
\qianru{*************Please introduce some basic features of datasets for causal discovery  here*********** }
One of the examples of real data used for Causal Discovery for Time Series is the US manufacturing growth data used by Entner et al. \cite{entner2010causal}. Growth  rates  of  US  manufacturing firms  in  terms  of  employment,  sales,  research and development expenditure, and operating income are included in this dataset. 
% \raha{please explain about the data, what is the groundtruth and how it is collected, in this section we do not focus on authors findings} %The authors claim to have found a link between employment and sales growth.

Human Motion Capture (MoCap) recordings dataset from CMU MoCap database contains data about joint angles, body position from two subjects. Tank et al.~\cite{tank2018neural} use this dataset in their Causal Discovery work. The dataset contains 54 joint angles over 2024 time points. Even though, there is no ground truth a causal graph can be created and compared with human anatomy.

An engine operating dataset is used by Xu et al.~\cite{xu2019scalable} for Causal Discovery. This dataset contains different attributes of engines like Fan speed, Cooling Outlet Temperature, Pressure, and Bleed Position over a period of six months. The dataset is created from 50 engines. According to the authors, the number of samples in this dataset exceeds 180,000. The dataset contains several causal relationships according to the authors.

Another air quality dataset is used by Pan et al.~\cite{pan2018hyperst} for causal discovery. This dataset includes the hourly concentration of pollutants. The pollutants include PM2.5, SO2, and NO. It also includes readings for related sensor data like temperature and wind speed. In total, 35 sensors are included. All of this data is collected in Beijing. 

Traffic Prediction dataset (METR-LA) is used by Pan et al.~\cite{pan2018hyperst} in the same work. This dataset contains four months' worth of sensor data from Los Angeles, California. 207 sensors are places for collecting this data. The location of each sensor in the form of GPS coordinates are also included in the dataset. TaxiBJ is also a similar dataset used in the same work. However, this dataset is collected from Beijing. Instead of GPS readings, this dataset contains the hourly inflow and outflow over a spatial grid. The inflow and outflow can be used in tandem with features of the Points of Interest and road networks for causal analysis according to the authors.

Flow Cytometry is a dataset proposed by Sachs et al.~\cite{sachs2005causal} and consists of nine different experimental conditions each performed on 800 observations. Each observation in this data corresponds to measurements of the concentration of biochemical agents in single cells. Each experimental condition in this data has a different external intervention which may act on several compounds at the same time. The first experimental setting contains pure observational data without any interventions.
This dataset is widely used in causal discovery algorithms such as~\cite{rothenhausler2015backshift}.

% \raha{this is a very famous dataset,  also this is not time series data, please add more references of time series papers using this data if you can find any}.

Stock Indices are a source of data used in Causal work. Rothenhausler et al. use NASDAQ, S\&P 500, and DAX indices for a period between 2000-2012 for their Causal Discovery work \cite{rothenhausler2015backshift}. They create 74 blocks of data. Each block represents 61 consecutive days. Upturns and Downturns in the indices represent the effects of a certain cause. 

\subsubsection{Synthetic Datasets for Causal Time-series}
Synthetic datasets are widely used in Causal Inference literature for time series. In this section, we taxonomize the datasets based on the type of synthesis and the properties of the resultant data. A summary of the synthetic models is presented in Table \ref{tbl:synthetic}. 

\qianru{Maybe we need to add a column named `model'. Autoregression and autocorrelation are not properties. The property of causal datasets they handled is time lagged (or something else). Also, non-linear model is not property. Please modify the table.}

\mk{I agree with Qianru, so I changed the ``Property" column name to ``Model" in the table. Modify it if you think it is not correct.}

\textbf{Autoregression/Autocorelation Models.}
Vector AutoRegressive (VAR) models are designed to create data where one component is a weighted sum of time-lagged components. VAR can be univariate or multivariate. Autocorrelated and Autoregressive models are used extensively in the literature for causal inference over time series~\cite{bica2019time, brodersen2015inferring, gong2017causal, runge1702detecting, schaechtle2013multi}. As an example, consider a multivariate VAR model of order one proposed by Papana et al.~\cite{papana2013simulation} where $X_1 \rightarrow X_2$ and $X_2 \rightarrow X_3$. Then,
\begin{align*}
x_{1,t} &= \theta_t \\
x_{2,t} &= x_{1,t-1} + \eta_t\\
x_{3,t} &= 0.5x_{3,t-1} + x_{2, t-1} + \epsilon_t
\end{align*}


$\theta_{t}$, $\eta_{t}$, and $\epsilon_{t}$ are Gaussian white noise processes. 


Sometimes, it is important to model a treatment in our simulation as well. Kerman et al.~\cite{kerman2017estimating} use a model where treated and untreated units are taken into consideration:
\begin{multline*}
	X_{i,t}=\beta_{0,t}+\beta_{1,t}X_{i,pre}+\beta_{2,t}Z_{i,t}\\+T_i(\mu_{0,t}+\mu_{1,t}X_{i,pre}+\mu_{2,t}g_i) +v_{i,t}
\end{multline*}
Here, $X_{i, pre}$ is a pre-period covariate, $g_i \in \{0,1\}$ is a group membership variable, $Z$ is the time-varying covariate and $T_i \in \{0,1\}$ is the treatment indicator. The $\beta$ values are decided based on a random walk over a state space. 


\newline
\textbf{Confounding/Common-cause Models.}
One of the concerns in causal literature is the effect or discovery of confounders. Thus, in order to model them, there are several approaches in the literature. 

Huang et al. use simulated datasets with a common cause and common effect \cite{huang2015fast}. The datasets contain noise variables and causal variables over time. Let $e(t)$ be the value of a variable $e$ at time $t$. Let $c$ represent the variable which causes $e$. Then:
$$
e(t)=\sum_{c\in X}\sum_{i=1}^{n}I(c, e)
$$
where $n=|T(c)\cap[t-s, t-r]|$ and $I(c, e)$ is the impact of $c$ on $e$. 

% \remove{Remove this sentence after you modify the table. There are various other works where confounding is modelled. We mention a non-linear model with confounding in the next section. }

\textbf{Non-Linear Models.}
Since many real-world systems are non-linear, there are works which try to simulate non-linear systems to evaluate their approach. 
An example of non-linear model is the simulation used by Papana et al.~\cite{papana2013simulation}. In their work, they simulate a tri-variate system with linear($X_2 \rightarrow X_3$) and non-linear($X_1 \rightarrow X_2$, $X_1 \rightarrow X_3$) relationships:


\begin{align*}
   	x_{1,t} &= 3.4 x_{1, t-1} (1-x_{1, t-1})^2 \exp(-x_{1,t-1}^2)+0.4\epsilon_{1,t} \\
   x_{2,t} &= 3.4 x_{2, t-1} (1-x_{2, t-1})^2 \exp(-x_{2,t-1}^2)+0.5x_{1,t-1}x_{2,t-1} \\ &{\ \ \ }+ 0.4\epsilon_{2,t}\\
   x_{3,t} &= 3.4x_{3,t-1}(1-x_{3,t-1})^2exp(-x_{3,t-1}^2)+0.3x_{2,t-1}\\&{\ \ \ }+0.5x_{1,t-1}^2+0.4\epsilon_{3,t}
\end{align*}

where $\epsilon_{i,t}$, $i=1,...,3$ are Gaussian white noise processes.

There are various other works which use non-linear models of data~\cite{lowe2020amortized}.
\newline
\textbf{Dynamic Models.}
Some models try to simulate a situation where the dependence of the variables vary over time in a non-linear and non-exponential manner. An example is the model used by Li et al.~\cite{li2018estimating} where there is a sinusoidal dependence:
\begin{multline*}
	X_t = \cos(X_{t-1} + X_{t-4}) + \log (|X_{t-6} - X_{t-10}| + 1) + \epsilon_t
\end{multline*}

For treatment effects, one of the examples of a model used in literature is defined as follows~\cite{kerman2017estimating}:
\begin{multline*}
	X_{i,t} = \beta_{0,t} + \beta_{1,t}X_{i,pre} +\beta_{2,t} Z_{i,t} + T_i\mu_{i,t}\cos(X_{i,pre}) +v_{i,t}
\end{multline*}
where $Z$ is the time-varying covariate, $v_{i,t}$ is the noise, $X_{i,pre}$ is the pre-treatment covariate, $T_i$ is the treatment indicator and $\mu_{i,t}$ represents the state.
\newline
\textbf{Chaotic Models.}
Choaticity is the ability of a model to deviate over different values of its hyperparameters. Chaoticity is usually expressed in terms of a Lorenz model. One of the examples of such a model which is also non-linear with $X_1 \rightarrow X_2$ and $X_2 \rightarrow X_3$ can be expressed as follows~\cite{papana2013simulation}:
\begin{align*}
\dot{x}_1 &= 10(y_1 - x_1) \\
\dot{x}_2 &= 10(y_2-x_2) + c(x_1 - x_2) \\
\dot{x}_3 &= 10(y_3 - x_3) + c(x_2 - x_3) \\
{\ }\\
\dot{y}_1 &= 28x_1-y_1-x_1z_1 \\
\dot{y}_2 &= 28x_2-y_2-x_2z_2 \\
\dot{y}_3 &= 28x_3-y_3-x_3z_3 \\
{\ }\\
\dot{z}_1 &= x_1 y_1 - 8/3 z_1 \\
\dot{z}_2 &= x_2 y_2 - 8/3 z_2 \\
\dot{z}_3 &= x_3 y_3 - 8/3 z_3
\end{align*}
where $c$ is the coupling strength. Variations of the Lorenz model is used in other places in causal inference for time series. The Lorenze-96 model is used in the work by Khanna et al.~\cite{khanna2019economy} where the authors mention it as a popular model for climate science.


\begin{comment}

\subsection{Datasets}
\raha{Anique: For the next week meeting (August 31st) Please prepare a table of all datasets for both causal discovery and causal treatment effect estimation along with their descriptions and references to the papers that have used them in their experiments}

\remove{Also for every synthetic data please put the description in a word document and send them to me. You can also take screen shots of equations if you do not wanna write them down}

\subsubsection{Time Series Data}
\remove{You can write it as one of the most common datasets used in time series literature can be obtained from UCR repo the then explain a bit about the datasets} \cmt{resolved}
In one of the more comprehensive surveys on time series models, Fawaz et al.\cite{fawaz2019deep} use 97 time series datasets to evaluate 8,730 deep learning models. The datasets in this study are taken from two time series dataset archives. One of the archives is the UCR Time Series Classification Archive \cite{UCRArchive2018} while the second archive is the one associated with Multivariate Time Series Classification with Learned Discretization \cite{Baydogan}. The UCR time series dataset is used in various other publications\cite{bagnall2015}\cite{xing2010brief}.

The UCR archive consists of several time series datasets. These datasets represent a classification problem. Thus, there is a class label for each item in every dataset in the archive. The length of the time series for each class in a single dataset is the same. Additionally, the classes are independent i.e. something that needs to be classified cannot occur in multiple classes in the ground truth\remove{classes or data points}\cmt{The authors only say that the classes are independent so I cannot make the claim about data points. clarification needed}. There are over 120 datasets in the archive. The intent of the authors is that instead of cherry-picking datasets to make claims about a time series approach, researchers should use all the datasets in the archive to ensure robustness of their approach\cite{UCRArchive2018} \remove{reference? and is it doable to do so?}\cmt{Added reference and clarification.}. Even though, it is possible to use a few datasets from the archive, the authors highly discourage researchers to do so. The authors provide three benchmarks\remove{comparing what? do you mean benchmarking?}\cmt{yes, fixed}: Euclidean Distance, Unconstrained DTW and Constrained DTW with learned warping width. 
\remove{Are these to archives only datasets used in time series analysis? are only datasets available are for classification? how about other approaches} \cmt{No, these are some of the most common ones. The UCR dataset can technically be used for non classification analysis as well because it does contain the series. I have added a paragraph mentioning datasets from another time-series survey} 

There are many other time series datasets in use apart from the ones included in the UCR archive. For	example, Real/Synthetic Yahoo Network traffic, Synthetic Yahoo Services with Seasonality,  Synthetic Yahoo Services with Changepoint Anomalies and NYC Taxi Dataset are recommended by Braei et al. \cite{braei2020}.

\subsubsection{Causal Time Series Data}
\qianru{\remove{If you agree, please refer to the following steps:}}

Traditional time series is not suitable for causal time series tasks. The reason is that there are several assumptions that are made about the data for causal analysis that we have already mentioned in Section \ref{sec:causal_background}. There are some differences between causal treatment effect estimation and causal discovery task. 

\qianru{\remove{traditional time series is not suitable for causal time series tasks. The reson is a)xxxx,b)xxxx}}



\qianru{There are some differences between the causal treatment estimation task and causal discovery task, due to xxxx. But the dataset of causal time series is scare, because xxx}

\qianru{For the causal treatment task, the dataset should contain some treatments and the time when the treatments are treated. The groundtruth is xxxx}

\qianru{For the causal discovery task, we need to xxxx}


Causal time series data is usually very scarce \remove{what are the main problems exactly? please explain}\cmt{Added more explanation}, so researchers tend to use synthetic data for evaluation quite often \cite{lowe2020amortized}\cite{hyttinen2016causal}\cite{gong2017causal}\cite{kleinberg2013causal}\remove{add some references} \cmt{Added}. The main problem here is that since causal frameworks are based on a set of assumptions, the data that we use to evaluate the causal models also have to follow the assumptions. Unfortunately, only a small subset of the time series data available to us checks all the boxes. For example, all for the datasets in the UCR archive are not i.i.d. datasets(An assumption which comes with some causal inference methods we have mentioned in this survey). \remove{this part is vague. please explain more?}\cmt{Added a sentence to clarify}

Since much of the causal time series data that does exist tends to be small, it is a common practice to construct\remove{train and test?}  a synthetic data model and see how it performs on realistic finite samples\cite{runge2018causal}\cite{gong2017causal}\cite{kleinberg2013causal}\cite{soleimani2017treatment}\cite{entner2010causal}. \remove{THis does not make sense, why should they only validate it on real data? and also I couldn't find this claim in the cited paper could you please quote that part here so that we could have a better understanding?}\cmt{First, I did not claim that \textbf{only} real data can be used for validation. Secondly, the claim is that it is a common practice to use simulated data for training. This has been the case for \textbf{all} the papers so far. The cited paper is an example. I have included more references. Third, this is mentioned in several papers to explain why they are using simulated data. One example where this is explicitly mentioned is \cite{runge2018causal} where they say: "Ideally, we would like to compare different methods on a data sample where the underlying causal truth is known or evaluate methods by experimentally manipulating a system, ... Since both of these options are mostly not available, an alternative is to construct synthetic model data where the underlying ground truth is known. These can then be used to study the performance of causal methods for realistic finite sample situations."} \remove{this claim is not equivalent to what we claim in the paper, it just simply says that due to the lack of real world data we test our models on the synthetic data}. This is because training usually involves looking at a large number of samples in order for the model to learn. Once the model is trained, it can be used on real data to see how it performs. Synthetic data is also capable of emulating do-experiments which is beneficial for training\cite{runge2018causal}. \remove{how do they make sure that the generalization error is bounded}
\remove{please elaborate more}\cmt{They use Gaussian Process. Added}

Since both simulated and real data are used across the publications related to causal time series analysis, we can look into both these categories in further detail.\\

\textbf{Real Data}.
\remove{the transition is too sudden, this part needs to be re organized}\cmt{fixed}
Real-world data for causal analysis can be either something that comes from a carefully crafted experiment or it can be observational data. 

In time series analysis, one of the most common datasets is the MIMIC II/III database\cite{johnson2016mimic}\cite{bica2019time}. This is a database create by MIT Lab for Computational Physiology. According to its website, it contains health data for approximately 60,000 people. This database consists of information about patients and caregivers in an Intensive Care Unit(ICU). Other than information about the patients status like laboratory measurements the database also contains temporal information like time of dialysis or insertion of lines. The MIMIC III database is an improvement and extension of the MIMIC II database where some of the inconsistencies were fixed and additional data was added \raha{anything specific?}\cmt{Here is the quote from the website: "MIMIC-III is an extension of MIMIC-II: it incorporates the data contained in MIMIC-II (collected between 2001 - 2008) and augments it with newly collected data between 2008 - 2012. In addition, many data elements have been regenerated from the raw data in a more robust manner to improve the quality of the underlying data." I tried to summarize it. There are additionally table fieldname and columns that were mentioned. I tried to summarize this. Can you please clarify what type of specifics should be mentioned?}. Thus, older publications may refer to MIMIC II, whereas, recent ones might mention MIMIC III.

\raha{please reorganize, we care more about the data used than the papers which are using the data, also there are other datasets available such as engine operating data please try to have all used datasets}There are several other small real-world datasets used in multiple causal analysis publications. Entner et al.\cite{entner2010causal} use growth rate of US manufacturing firms from 1973-2004. Schaechtle et al.\cite{schaechtle2013multi} use Diabetes data to figure out if Insulin and Glucose are related. The two-variable dataset\cite{mooij2016distinguishing} contains multiple sets of causal data with two series of covariates e.g. Ozone and Radiation, a causal model can be evaluated based on whether it identifies whether Ozone is responsible for Radiation or vice versa.


\textbf{Synthetic Data}. Since synthetic data is very popular for training a causal model, there are publications which advise on how to create such data. One of the challenges while creating simulated data is to make sure that is resembles real data\cite{mooij2016distinguishing}. Mooij et al. \cite{mooij2016distinguishing} outline an approach for generating simulated causal data where randomly generated functions are used in conjunction with randomly generated distributions for the causes, effects and confounders. Gaussian noise is added to the resultant values. Finally, one of four kinds of perturbations are added: unperturbed, discretized, undiscretized, and small noise.
There are several other approaches for simulating causal time series. Kleinberg et al.\cite{kleinberg2013causal}\cite{kleinberg2011logic} use the Fama-French daily factors to simulate stock exchange data. Another notable datasets is the Kuramoto Model Simulation used by \cite{lowe2020amortized} where the neurons in the brain of a Parkinson's patient are simulated.
Lets take an example of a data simulation model from Mooiji et al. Let $p_{E_X}$, $p_{E_Y}$, and $p_{E_Z}$ be randomly generated noise distributions. Let $f_X$, $f_Y$, and $f_Z$ be randomly generated functions representing the causal mechanisms. Let X be the cause of Y and Z be the confounder. Then:
\begin{align*}
E_X &\sim p_{E_X},\ E_Y \sim p_{E_Y},\ E_Y \sim p_{E_Y} \\
X &= f_X(E_X, E_Z)\\
Z &= f_Z(E_Z)\\
Y &= f_Y(X, E_Y, E_Z)\\
\end{align*}

\remove{Are you sure this is designed for time series? I know for a fact that they use this approach to sample from i.i.d data please double check}\cmt{Yes, \cite{gong2017causal} uses the simulated data from this paper and cite them.}

Here Gaussian Process is used to sample a random function which is used for $E_X$, $E_Y$, and $E_Z$. The causal mechanisms are also generated using the Gaussian Process.

\remove{Is there any formulas? could you please explain one data generation process in detail?}\cmt{Added an example. Different papers use different approaches. I have included one as an example.}

\end{comment}

==> Evaluation/metrics.tex <==
\subsection{Evaluation Metrics}
\qianru{Please merge the metrics for time series and metrics for causal inference. I think it is not necessary to present them separately. Because some metrics for time series are also used in causal inference.}

\qianru{The section should be consistent with the previous sections.
Please introduce the metrics for causal estimation and causal discovery separately.}

\qianru{please introduce what we need to evaluate in the problem before presenting the metrics for each problem.}
\qianru{Metrics for causal estimation: 
We need to evaluate the prediction results after the treatment.
Introduce some metrics for time series are also used in causal inference: Accuracy.
Give some metrics only for causal estimation if we have.
}

\qianru{Metrics for causal discovery:}


In this section, we look at different metrics used in the literature for measuring how well a model performs. Since there are different approaches based on the type of analysis we want to fulfill, there are multiple metrics in use.

\qianru{There are so many metrics only for time series.  Please select some metrics related to causal inference.}

\subsubsection{Time Series Metrics}
There are multiple time-series metrics used in the literature.  Here we discuss some of the commonly used ones. We also go over the two most common benchmarks for time series: Euclidean distance and Dynamic Time Warping.

\textbf{Accuracy.}
One of the common metrics for validating time series classification models is by looking at the accuracy of the models. The accuracy is simply the percentage of samples that are correctly classified. Accuracy is especially popular in literature where neural network models are being compared~\cite{fawaz2019deep, lines2016hive}.

\textbf{Mean/Median Error.}
There are several variations of errors used in time series literature, particularly for time series forecasting~\cite{hyndman2006another} such as (Root) Mean Squared Error, Mean/Median Absolute Error, Mean/Median Absolute Percentage Error, Symmetric Mean/Median Absolute Percentage Error, Median Relative Absolute Error, Geometric Mean Relative Absolute Error, and Mean Absolute Scaled Error. All of these are intended to measure the differences between the forecasted time series and the ground truth. 

\textbf{K-fold Cross-validation.}
In k-fold cross-validation, the data is divided into k partitions. Each partition is first used as a test set and the remaining data is used as a training set. The model is trained on the training data and the accuracy is measured on the test data. The test accuracy is recorded and the trained model is discarded for the next iteration where the next partition is used as a test set. There are various ways to partition the data into folds. One of the ways is to re-sample with stratification such that the distribution of the original classes is preserved~\cite{bagnall1602great}. 


\textbf{Longest Common SubSequence.}
A common metric that is popular among text series is the Longest Common Subsequence (LCSS)~\cite{bagnall1602great}. In this metric, when two sequences are being compared, we find an ordered subset from both the sequences such that the length of the subsets is maximized and the intersection is an empty set.

\textbf{Edit Distance with Real Penalty.}
In this metric, the distance between the two series is measured by looking at the number of operations required to change one series into the other series. One of the variables used here is $\sigma$ which is the Sakoe-Chiba window size~\cite{sakoe1978dynamic}. A distance matrix is created which stores the distances between the two time series across multiple time points inside the time window. Gaps between points are penalized according to a user-provided reference value~\cite{chen2004marriage}.


\textbf{Move Split Merge.}
The Move Split Merge (MSM) metric is similar to Edit Distance metric~\cite{bagnall1602great}. Given two sequences, it calculates the number of operations in terms of either move, split, or merge to convert one sequence into the other sequence. The move operation replaces one value with another. The split operation creates a duplicate of the value adjacent to the original value. Finally, the merge operation merges two adjacent points with the same value with a single point.


Among time series literature, Euclidean distance and Dynamic Time Warping are used as popular benchmarks to compare models.

\textbf{Euclidean Distance.}
One of the simplest benchmarks for time series is the Euclidean Distance (ED). Given two series, the square root of the sum of squared distances between each time step is the euclidean distance. 

\begin{definition}
	Euclidean Distance - Given two time series $X_{1} = (x_{1}, ..., x_{t})$ and $X_{2} = (x^{'}_{1}, ..., x^{'}_{t})$, the euclidean distance between $X_{1}$ and $X_{2}$ is given by $\sum_{i=1}^{n} (x_{i} - x^{'}_{i})^{2} $	
\end{definition}

\textbf{Dynamic Time Warping.}
Another common metric to measure the similarity between two temporal series is Dynamic Time Warping.
\begin{definition}
	Dynamic Time Warping~\cite{berndtDTW1994} - Given two time series $X_{1} = (x_{1}, ..., x_{t})$ and $X_{2} = (x^{'}_{1}, ..., x^{'}_{t^{'}})$, to find the DTW distance, a matrix M of size t by $t^{'}$ is constructed which consists of the distance between a given time stamp value of $X_{1}$ with give time stamp of $X_{2}$. Thus, the ith row and jth column of matrix M represented by $m_{ij}$ consists of the distance between the points $t_{i}$ and $t^{'}_{j}$, denoting the alignment between $t_{i}$ and $t^{'}_{j}$. The distance between two points is typically chosen to be a euclidean distance. A contiguous set of matrix elements, denoted as the warping path W, where the kth element is $w_{k} = (t_{k}, t^{'}_{k})$ and the warping path W = $w_{1},w_{2},..., w_{k},..., w_{K} $, where max(m,n) $\leq$ K $<$ m + n -1. For a warping path to be valid the following constraints need to be satisfied:- ($t_{1}, t^{'}_{1}$) = 1; ($t_{K}, t^{'}_{K}$) = (m,n); $0 \leq t_{k+1} t_{k} \leq 1 $; and $0 \leq t^{'}_{k+1} t^{'}_{k} \leq 1 $. The DTW distance is the warping path, among exponentially possible warping paths that minimizes the total distance subject to the constraints mentioned above.
\end{definition}

The most common metric in this regard is the 1-NN classifier with the DTW distance measures~\cite{hui2008}. Jeong et al. defined weighted penalties ~\cite{Jeong2011} based on the warping distance to reduce the warping horizons. Another similar distance measure is proposed where the transformation of one series to another series is defined using new operations move, split and merge ~\cite{stefan2013}. The distance measured described before are based on the first-order differences. \mk{Did you intend to say ``different domains"? I do not understand the sentence that follows:} Other distance measures also include distances from the difference domain. Batista et al.~\cite{batista2014} propose a weighting method to take into account complexity differences in time series. The measure of complexity is chosen as the sum of squares of the first difference. A weighted combination of the original time series and the first-order differences are proposed by Górecki et al.~\cite{gorecki2013} referred to as DDTW. The same authors also combined DDTW with three non-isometric transforms: sine, cosine, and Hilbert transform~\cite{gorecki2014}.

\begin{comment}
\textbf{Piecewise Aggregate Approximation(PAA)}\newline
Piecewise Aggregate Approximation(PAA) \cite{keogh2001dimensionality} reduces the raw time series dimensions by taking average value of fixed length intervals of the time series. For a time series X = ($x_{1}, x_{2}, ... , x_{m} $) with a dimension of m, the compressed time series $\hat{X}$ = ($\hat{x}_{1},\hat{x}_{2}, ..., \hat{x}_{n} )$ with a dimension n is obtained by :- 

\begin{equation}
\hat{x}_{k} = \frac{1}{e_{k} - s_{k} + 1} \sum_{i = s_{k}} ^{e_{k}} x_{i}
\end{equation}

\textbf{Symbolic Aggregate Approximation}\newline
Symbolic Aggregate Approximation(SAX)~\cite{Lin2003},a method  to convert a numeric time series representation into a symbolic representation, builts upon the PAA framework by dividing the time series into equal segments, averaging, and  mapping every value to a string. To map the values to a string equiprobable regions are created from the distribution space, and each region is represented by a symbol. The PAA transformed time series $\hat{X}$ is converted to a string representation S = ($s_{1}, ...,s_{w}$).
Lin et al.~\cite{lin2012} applies Symbolic Aggregate Approximation (SAX) \cite{Lin2003} based on PAA~\cite{keogh2001dimensionality} to the windows to get a word representation for each window. A count histogram is created over the word distribution of the time series and the euclidean distance between the count histograms are used as a distance measure for the 1-NN classifier. Instead of creating the word distributions over the time series, Senin et al.~\cite{senin2013} creates word distributions over classes using tf-idf to weigh the distribution, using SAX representation and the vector space model in Information Retrieval.
\end{comment}


\begin{table*}[h!]
\label{tab:cmetrics}
\begin{center}

\begin{tabular}{| >{\centering\arraybackslash}m{0.25cm}|l|m{5.4cm}| >{\centering\arraybackslash}m{5.2cm}| >{\centering\arraybackslash}m{0.25cm}| >{\centering\arraybackslash}m{0.25cm}| >{\centering\arraybackslash}m{0.25cm}| >{\centering\arraybackslash}m{0.25cm}|} 
\hline
   & \textbf{Metric Name}   & \textbf{Notions} & \textbf{Definition} & \rotatebox[origin=c]{90}{\textbf{Correctness}} & \rotatebox[origin=c]{90}{\textbf{Robustness}}  & \rotatebox[origin=c]{90}{\textbf{Comparative}} & \rotatebox[origin=c]{90}{\textbf{Significance}}  \\ 
\hline\hline

1  &  TPR & \multirow{2}{=}{{Let $G = (V, E_M)$ be the causal graph infered by the model, where $V_M = \{v_1, v_2, ..., v_n\}$ represent the covariates (including time-lagged) and $E_M$ represent the edges between the covariates if there is a direct causal dependence. Similarly, let $G' = (V, E_{GT})$ represent the covariates and the edges in the ground truth. Let $E = \{e_1, e_2, ..., e_m\}$ represent all possible edges between $V$.}} &    $TPR = \mathlarger{\sum}_i \frac{e_i}{|E_{GT}|},\ e_i \in E_M \cap E_{GT}$     &     \cmark         &            &             &               \\[5em]
\cline{1-2}\cline{4-8}
2  & FPR        &         &  $FPR = \mathlarger{\sum}_i \frac{e_i}{|E - E_{GT}|},\ e_i \in E_M \backslash E_{GT}$      &   \cmark          &            &             &               \\ [5em]
\hline
3  & MSE           &   Let $T$ be the inferred transition matrix and $A$ be the adjacency matrix for the ground truth.        &   $MSE = \frac{1}{|T|} \sum (T-A)^{\circ 2} $      &   \cmark          &            &             &               \\ 
\hline
4  & KL-Divergence &   Let $P$ be the distribution for the p-values in the test data and $Q$ be a uniform distribution         & \  $D_{KL}(P||Q) = \mathlarger{\sum}_x P(x) \ln \frac{P(x)}{Q(x)}$      &             &      \cmark      &             &               \\ 
\hline
5  & AUPC          &     Let $T(\sigma)$ be the TPR of the model for a particular value of $\sigma$       &       $AUPC = \int_\sigma T(\sigma)$  &             &      \cmark      &             &               \\ 
\hline
6  & Precision     &   Let $TP$ and $FP$ denote the True Positive and False Positive, respectively.         &   $	Precision = \frac{TP}{TP + FP} $      &     \cmark        &            &             &               \\ 
\hline
7  & Recall        &     Let $TP$ and $FN$ denote the True Positive and False Negative, respectively.       &     $	Recall = \frac{TP}{TP + FN}	$    &     \cmark        &            &             &               \\ 
\hline
8  & F1-Score      &     Let $P$ and $R$ be the precision and recall, respectively       &    $	F_1 = \frac{2PR}{P + R}	$    &   \cmark          &            &             &               \\ 
\hline
9  & F-Test        &    Let $RSS_0 = \sum_{t=1}^T \hat{e}_t$ and $RSS_1 = \sum_{t=1}^T \hat{u}_t$, where T is the length of the time series, $\hat{e}_t$ and $\hat{u}_t$ is the time dependent error for the null hypothesis and the alternative hypothesis, respectively.     &  $F = \frac{(RSS_0 - RSS_1)/p}{RSS_1/(T-2p-1)}$       &             &            &       \cmark      &       \cmark        \\ 
\hline
10 & Unpaired T-Test        &    Let $\bar{x}_1$ and $\bar{x}_2$ be the means of two sequences. Let $s_1$ and $s_2$ represent the standard deviation of the sequences. Let $n_1$ and $n_2$ represent the cardinalities of the sequences.        &     $utt = \frac{\bar{x}_1 - \bar{x}_2}{\sqrt{(\frac{1}{n_1}+\frac{1}{n_2})(\frac{(n_1-1)s^2_1 + (n_2-1)s^2_2}{(n_1-1)+(n_2-1)})}} $    &             &            &             &    \cmark           \\
\hline
\end{tabular}
\caption{Causal time series metrics and their definition.}
\end{center}

\end{table*}



\subsubsection{Causal Time Series Metrics}
\mk{There are a lot of definitions in between the paragraphs! Maybe, instead of this, if we provide a table defining the metrics would make it much more structured. }


In this section, we look at different metrics used in the literature for causal discovery and causal inference with time series. The metrics are usually selected based on the type of causal inference. For example, causal discovery research mainly involves finding the causal relationships~\cite{entner2010causal, runge1702detecting}, so the metrics involved in this type of approach might be a measure of correctly identified relationships. In contrast, works related to causal effect estimation might prefer metrics which give better feedback on how successful a model was in estimating a specific value. 
% \begin{table}[]
%     \centering
%     \begin{tabular}{|c|c|}
%         \hline
%          & \textbf{Metric} \\ \hline
%          \textbf{Correctness} & TPR, FPR, FNR, MSE  \\ \hline
%          \textbf{Robustness} & KL-divergence, AUPC \\ \hline
%          \textbf{Comparative} & AUROC, T-Test \\ \hline
%          \textbf{Significance} & T-Test, F-Test \\ \hline
%     \end{tabular}
%     \caption{Commonly used metrics}
%     \label{tab:metrics}
% \end{table}

Since causal discovery methods try to reconstruct the causal relationships, binary metrics which count the number of correct classifications are popular in this area. Some commonly used causal discovery metrics include True/False positive rate (TPR/FPR), Mean Squared Error, Area Under the Power Curve, Area Under the Receiver Operator and F-Test. 

For causal effect estimation, the metrics which are used, give us information about how well the estimation compares to the ground truth. Common metrics for this area include Mean Squared Error, T-test, and F-test. Even though, causal discovery appears to have a very different objective than causal effect estimation, there are metrics which are common for both.

 
% \remove{what are the definitions? If you are gonna define them later you need to say it explicitly? also it would be better not to have them listed and casually mention them in the text}
% %\begin{itemize}
% %   \item True Positive Rate(TPR)/False Positive Rate(FPR)
% %   \item Mean Squared Error(MSE)
% %  \item Kullback-Leiber divergence 
% %   \item Area Under the Power Curve(AUPC) 
% %   \item Area Under the Receiver Operator(AUROC)
% %   \item F-Test
% %\end{itemize}
% \remove{please put the mathematical definitions and write the accurate definition for each metric}\cmt{added}


\textbf{True/False Positive Rate}.
Multiple publications~\cite{hyttinen2016causal,runge1702detecting,runge2018causal,schaechtle2013multi} use TPR/FPR to evaluate the reconstructed causal relationships. This involves looking at pairs of nodes. Some works extend the idea of TPR/FPR to be a bit more involved. Entner et al.~\cite{entner2010causal} propose three metrics for evaluating a causal model: direct-cause, ancestor, and pairwise scores. Each of these scores measures the percentage of pairs to make a ternary decision (correct, incorrect, or don't know). In the direct-case score, the percentages of nodes that directly affect other nodes are measured. In the ancestor score, the percentage of ancestor node/node pairs are measured. Finally, in the pairwise scores, the percentage of variable pairs is measured across lag, where one variable affects another.

\raha{please cite the papers which have used a specific papers, we need to know which papers have used a specific metric.}\mk{ Not provided.}

% \begin{definition}[True/False Positive Rate]
% Let $G = (V, E_M)$ be the causal graph infered by the model, where $V_M = \{v_1, v_2, ..., v_n\}$ represent the covariates (including time-lagged) and $E_M$ represent the edges between the covariates if there is a direct causal dependence. Similarly, let $G' = (V, E_{GT})$ represent the covariates and the edges in the ground truth. Let $E = \{e_1, e_2, ..., e_m\}$ represent all possible edges between $V$.

% The true positive rate is defined as:
% \begin{equation}
%     TPR = \mathlarger{\sum}_i \frac{e_i}{|E_{GT}|},\ e_i \in E_M \cap E_{GT}
% \end{equation}

% Similarly, false positive rate is defined as:
% \begin{equation}
% \label{eq:fpr}
%     FPR = \mathlarger{\sum}_i \frac{e_i}{|E - E_{GT}|},\ e_i \in E_M \backslash E_{GT}
% \end{equation}

% \end{definition}

\textbf{Mean Squared Error.}
This metric is used to evaluate works in causal discovery and causal reasoning alike. In Causal Discovery for Temporally Aggregated Time Series~\cite{gong2017causal}, the authors construct a transition matrix to represent the causal graph. Here, the MSE between the distance from the transition matrix to the ground truth is used to evaluate the causal relationships inferred by the proposed model. 

% \begin{definition}[Mean Squared Error (MSE)]
% Let $T$ be the inferred transition matrix. Let $A$ be the adjacency matrix for the ground truth. Then, the MSE is defined as:
% \begin{equation}
% MSE = \frac{1}{|T|} \sum (T-A)^{\circ 2}    
% \end{equation}
% \end{definition}

MSE and its variations (Root Mean Squared Error~\cite{pan2018hyperst}, Normalized Root Mean Squared Error~\cite{soleimani2017treatment}) are used commonly in causal effect estimation literature~\cite{bica2019time,kerman2017estimating}. In general, MSE is used to compare the inferred series with the ground truth series by taking the average of the squared differences at each time step. 

\textbf{KL-Divergence.}
Runge et al.~\cite{runge2018causal} suggested the KL-Divergence as a method of evaluation. KL-divergence isn't a metric in the same sense as the previously mentioned ones. The authors propose that using KL divergence can help us see how well the tests are calibrated by looking at the distribution of p-values. If a test is calibrated well, the p-values have to ideally be uniformly distributed. KL-divergence can be used as a measure of finding how close the test distribution is to a uniform one. 

% \begin{definition}[Kullback-Leiber (KL) Divergence]
% Let $P$ be the distribution for the p-values in the test data and $Q$ be a uniform distribution. Then KL-divergence is defined as:
% \begin{equation}
% D_{KL}(P||Q) = \mathlarger{\sum}_x P(x) \ln \frac{P(x)}{Q(x)}
% \end{equation}
% % \cmt{The authors of the paper only mention this in words and there are multiple ways to interpret what they mean. For both KL-divergence, AUPC}
% \end{definition}
\begin{aniq}
	I am not completely sure about the AUPC metric. I suggest that the reviewers ensure that my understanding is correct.
\end{aniq}
\textbf{Area Under the Power Curve.}
Runge et al.~\cite{runge2018causal} suggest using Area Under the Power Curve to compare different models. Here the curve is created by plotting the True Positives against $\sigma$, where $\sigma$ is the coefficient for added noise. The higher the value of $\sigma$, the more noise that is added, and the worse the model performs. Thus, over all the values of $\sigma$, a more robust model would have a higher AUPC. 

\mk{Where did you find the definition of AUPC? I need to go over that instead of this paper. In the cited paper, they only mentioned that this metric is used to calculate the TP without providing any definitions.}
% \begin{definition}[Area Under the Power Curve]
% Let $T(\sigma)$ be the TPR of the model for a particular value of $\sigma$. The AUPC is defined as:
% \begin{equation}
%     AUPC = \int_\sigma T(\sigma)
% \end{equation}
% \end{definition}

%% TODO Add causal equations where sigma is used from the paper
\textbf{Area Under the Receiver Operator Curve.}
This measure is one of the most popular metrics for Causal Discovery~\cite{haufe2010sparse,khanna2019economy, lowe2020amortized,wunonlinear,xu2019scalable}. The Receiver Operator Characteristic (ROC) is defined as a ratio of TPR and FPR. The ROC curve is created by iterating over the cut off for classification and recording the TPR against the FPR. The area under the ROC curve (AUROC) is a useful metric to judge a model. The higher the value of this metric, the better the model. The area under this curve can be used to compare different models.

\textbf{Area Under the Precision Recall Curve.}
Area Under the Precision Recall Curve (AUPR) is another metric used in literature~\cite{tank2018neural,xu2019scalable}. This metric relies on precision and recall. Similar to the AUROC, this metric measures the area under the Precision-Recall curve.

% \begin{definition}[Precision]
% $$	Precision = \frac{True\ Positives}{True\ Positives + False\ Positives}
% $$
% \end{definition}

% \begin{definition}[Recall]
% 	$$	Recall = \frac{True\ Positives}{True\ Positives + False\ Negatives}
% 	$$
% \end{definition}

Precision and Recall can also be used to calculate the F1-score~\cite{arnold2007temporal}.

% \begin{definition}[F1-score]
% 	Let $P$ and $R$ be the precision and recall respectively. The F-1 score is defined as:
% 	$$
% 	F_1 = \frac{2PR}{P + R}
% 	$$
% \end{definition}

\textbf{F-Test.}
One approach to finding whether causality exists is the F-test~\cite{papana2013simulation}. This test can be used, for instance, to see if there is a granger causality between time series. Taking the example of bi-variate granger causality, we can construct a restricted and unrestricted equation and estimate the hyper-parameters using Ordinary Least Squares. 
\begin{definition}[F-Test]

Let $X = \{x_t, x_{t-1}, x_{t-2}, ... \}$ be one series. Let $Y = \{y_t, y_{t-1}, y_{t-2}, ... \}$ be another series. The null hypothesis is given by the restricted equation:
\begin{equation}
    x_t = c_1 + \sum_{i=1}^p \gamma_ix_{t-i} + e_t
\end{equation}
Where $p$ is the lag, $c_1$ is the intercept and $e_t$ is the time-dependent error.

The unrestricted equation represents the alternative hypothesis:
\begin{equation}
     x_t = c_2 + \sum_{i=1}^p \alpha_ix_{t-i} + \sum_{i=1}^p \beta_i y_{t-i} + u_t
\end{equation}
Where $p$ is the lag, $c_2$ is the intercept and $u_t$ is the time-dependent error.

Let $RSS_0 = \sum_{t=1}^T \hat{e}_t$ and $RSS_1 = \sum_{t=1}^T \hat{u}_t$, where T is the length of the time series. The F-test statistic is defined as:
\begin{equation}
    F = \frac{(RSS_0 - RSS_1)/p}{RSS_1/(T-2p-1)}
\end{equation}

\end{definition}

%% TODO Causal Reasoning Metrics
%% Most of the work in causal reasoning deals with estimating the effect. Thus, the metrics used for causal reasoning are mainly focus on how accurately the effect estimation is. Some commonly used metrics for causal reasoning are Type I/II rate, T-Test and Mean Squared Error.
%\begin{itemize}
%    \item Type-I/Type-II rate
%    \item T-Test
%    \item Mean Squared Error (MSE)
%\end{itemize}
\textbf{Type-I/II Error Rates.}
Type-I and Type-II rates are also commonly known as `False Positive Rate' and `False Negative Rate', respectively. The definition of false positive rate is given in Table \ref{tab:cmetrics}. \mk{The reference to the table is not showing correctly. } They are used similarly to TPR in causal discovery~\cite{huang2015fast}. 
% In causal effect estimation, instead of using edges, one of the ways this metric is used is by discretized along the time dimension~\cite{kleinberg2013causal} among covariates. These discretized covariates are used for calculating False Positives and False Negatives.
% \begin{definition}
% False Negative Rate is defined as:

% \mk{This was already defined in Definition 7}

% \begin{equation}
%         FPR = \mathlarger{\sum}_i \frac{e_i}{|E_{GT}|},\ e_i \in E_{GT} \backslash E_M
% \end{equation}
% \end{definition}
\begin{aniq}
	For the reviewers: Please verify if I have the correct understanding of \cite{kleinberg2013causal}
\end{aniq}
\mk{No, it is not correct as this measure was not used for the causal effect estimation in that paper! I will comment it out.}

\textbf{T-Test.}
The t-test is a metric used to compare two sequences. In their work on causal inference with rare time series data, Kleinberg et al.~\cite{kleinberg2013causal} use an unpaired t-test to determine the significance of a cause within a certain time-range. 
% \begin{definition}[Unpaired T-Test]
% Let $\bar{x}_1$ and $\bar{x}_2$ be the means of two sequences. Let $s_1$ and $s_2$ represent the standard deviation of the sequences. Let $n_1$ and $n_2$ represent the cardinalities of the sequences. The unpaired t-test($utt$) is defined as:
% \begin{equation}
%     utt = \frac{\bar{x}_1 - \bar{x}_2}{\sqrt{(\frac{1}{n_1}+\frac{1}{n_2})(\frac{(n_1-1)s^2_1 + (n_2-1)s^2_2}{(n_1-1)+(n_2-1)})}} 
% \end{equation}

% \end{definition}


\textbf{Structural Hamming Distance.}
Structural Hamming Distance (SHD) is another metric used for Causal Discovery~\cite{peters2013causal}. SHD can be used to compare a discovered causal graph with the ground truth. This metric uses three operations: edge insertions, deletions, and flips. The magnitude of this distance is determined by the minimum combinations of the three operations to convert one graph into the other one.






==> TimeSeriesModelling/TimeSeries.tex <==
Before we move on to causal methods for time series data, we want discuss some traditional approaches for time series data. Other surveys in the field[][][]  


 
  \subsubsection{Statistical Models for Time Series Analysis}
  \raha{In each subsection, we need to first explain what we are going to talk about and then have a list of models}
  \begin{enumerate}
       \item AutoRegressive Model(AR)
       It is a linear stochastic model where the current timestamp value $X_{t}$ is determined by a finite set of values from previous timestamps of length p and some error $\epsilon$. These models assume that the data is stationary. 
       
       Mathematically, $X_{t} = \sum_{i=1}^{p} a_{i}.X_{t-i} + c + \epsilon_{t}$ 
       
       The values of the coefficient $a_{i}$ and c can be approximated from the training data by solving the linear equations with least-squared regression. 
       
       \item Moving Average Model(MA) 
       
       In a MA Model the current timestamp observation $X_{t}$ is a linear combination of the prediction errors at the previous timestamps of length p. 
       
       Mathematically, $X_{t} = \sum_{i=1}^{q} a_{i}.\epsilon_{t-i} + \mu + \epsilon_{t}$, where ${\epsilon_{t}, ... , \epsilon_{t-q}}$ are the last q prediction errors.
       
       \item Autoregressive Moving Average Model(ARMA)
       
       In an ARMA(p,q) model, the value at current time instance is dependent on last p observations and q errors :-
       
        \begin{equation}
            X_{t} = \sum_{i=1}^{p}a_{i}.X_{t-i} + \sum_{i=1}^{q}b_{i}.\epsilon_{t-i} + \epsilon_{t} 
        \end{equation}
       
       The assumption is that ${X_{t}}$ is stationary.
       
       The main challenges in ARMA models are selecting the appropriate values of p and q. There are mainly 3 methods to do this - using correlograms, leave-one-out cross-validation, and the box-jenkins procedure \cite{boxjenkins1990}.
       
      \item ARIMA model
      
      ARIMA model is a generalization of the ARMA model with an additional parameter d which is the number of times the time series is differenced. This allows for working with non-stationary data unlike previous models such as ARMA. 
      
      For a time series ${x_{0}, ..., x_{T}}$ differencing is done as follows:- 
      
      \begin{equation}
          X_{i}^{'} = X_{i} - X_{i-d}, \forall i \in {1, ..., T}
      \end{equation}
       
      \item Simple Exponential Smoothing(SES) \cite{brown1956exponential}
      
      In SES an non-linear approach is used where the value at current time step depends on the previous time series data , with exponential weights assigned to each observation. Mathematically, 
      
     \raha{Equations need to be rewritten please check out my format}
      
          \begin{multiline}
                  X_{t+1} = \alpha X_{t} + \alpha(1-\alpha) X_{t-1} + \alpha(1-\alpha)^{2}X_{t-2} + ...  + \\ \alpha(1-\alpha)^{N} X_{t-N} 
          \text{ where }  \alpha \in [0, 1]
              
          \end{multiline}
      
    \item Double and Triple Exponential Smoothing(DES, TES) \cite{esm2002}
    
    This is an extension of SES for handling non-stationary data. In DES, an additional parameter $\beta $ is used for smoothing the trend in the series. Additionally, a extra parameter $\gamma$ is introduced in TES to control the influence of seasonality. 
      
       
       
       
   \end{enumerate}
   
   
      \anchit{Anomaly detection}
   \cite{Yairi01faultdetection} \ab{ proposes k-means clustering \cite{macqueen1967} methods for detecting anomalies in time series data. First the time series data is divided using sliding windows of length w and slide length y. Then k-means algorithm is applied on the sliding window vectors to learn k clusters. Each subsequence distance e from it's nearest centroid is computed using euclidean distance measure, and based on a threshold value $\sigma$ the window subsequence is classified as anomaly if e $>$ $\sigma$. Another clustering algorithm DBSCAN was used in \cite{Celik2011AnomalyDI} to find anomalies in temperature data. The dataset is split into sequences for every month and normalized using the mean and variance of the sequence. The points are classified as anomalies if it's neither a core point or a border point.}
   
    \anchit{Anomaly detection - neural networks}
   \ab{
   \cite{hyndman2014forecasting} proposes a Neural Network Autoregression Model(NNAR) which is modelled using the number of lagged time-series input p and and the number of hidden layers k, denoted as NNAR(p, k). For a time series, $x_{i} \in {X_{N}}$, the window length w, and the MLP function f the time series prediction $x^{'}_{t+1}$ is equal to $f(x_{t-w},..., x_{t})$. The number of predictions can be increased such that $(x^{'}_{t+1},...,x^{'}_{t+P_{w}}) = f(x_{t-w},..., x_{t})$ where $p_{w}$ is the number of timestamps predicted by the MLP. The error of predictions is used to detect an anomaly based on a threshold value determined from the training data.  
  \cite{chauhan2015} predicts electrocardiography signal health using a LSTM model and uses the prediction error probability distribution to find anomalous signals. \cite{malhotra2015} uses two stacked LSTM layers to predict the next l time-steps. The error value of each prediction is computed forming an error vector. A multivariate gaussian distribution is used to fit the error vectors using MLE, and for a timestamp based on the probability value and a threshold anomalous values are determined. Other sequence models such as Gated Recurrent Unit(GRU) is also used with time series.  \cite{wu2019local} uses stacked GRU's for time series anomaly detection, which is similar to the LSTM based models. \cite{sakurada2014} uses normal and denoising autoencoders to reduce the dimensionality of the time-series data for anomaly detection. The idea is that the distribution of normal and anomalous data is different in anomalous space, and thus the prediction error of the trained autoencoder can be used to detect anomalies. }
  
  
  \anchit{Anomaly detection}   
   \ab{
   \cite{stefan2015} uses Local Outlier Factor(LOF) clustering for time series data, which is based on kNN's than density estimation in DBSCAN algorithm. The time series is divided into subsequences using the sliding window technique, and the local outlier factor of subsequence is computed which is used to determine anomalous sequences based on a threshold value. \cite{DING201312} extended isolation forest techniques on time-series data by using a sliding window based representation of the time series and defining anomaly score based on the data points, window size and length of the i-tree. One class SVM(OCSVM) \cite{bernhard99} can detect anomalies when there is only one class in the training set using semi supervised learning. \cite{ma2003} uses time-delay embedding process to convert a time-series into a phase space so that OCSVM can be used. \cite{zhang2007} \cite{zhang2008} creates a sliding window subsequence and then projects the subsequence into a 2-D space before applying OC-SVM.  \cite{braei2020} uses Extreme Gradient Boosting(XGboost) as a regression model for time series forecasting and uses the error in prediction and error distribution based threshold to determine anomalies.}
   
     \anchit{ML based Classification}
   Clustering algorithms modified specifically for time series data has been proposed. An iterative and incremental version of k-means is proposed by called i-kMeans. Multi-resolution property of wavelets are are used to reduce the problem of initial cluster selection.
   
   %ARIMA 
   
     One of the earlier methods to model time-series data is the AutoRegressive Integrated Moving Average(ARIMA) model. The ARIMA models the time-series assuming three fundamental relationships between the time series - autoregressive, moving average and differencing \anchit{elaborate} . The Autoregressive(AR) component determines the value of a current timestamp $X_{t}$ from a finite set of values from previous timestamps of some length p and some error $\epsilon$. The number of previous timestamps used to determine the value of the current timestamp is called the order of autoregression.
   \anchit{the concept of auto regression needs to be defined also, ARIMA is generative?} - \anchit{It does try to model the relationship between different timestamps to learn the time series generation process, but not solely from a single model. It uses some statistical methods(e.g autocorrelation function) to make some assumption on the structure of the data} 
   \begin{equation}
       AR(p) =  \sum_{i=1}^{p} a_{i}.X_{t-i} + c + \epsilon_{t}
   \end{equation}
   
   where $a_{i}$ and p are the coefficient and the order of the AR model respectively.
   \anchit{do we really need moving average?} - \anchit{If we are mentioning ARIMA - moving average is one of the components of ARIMA}
   The moving average(MA) component models the value of a current timestamp $X_{t}$ as a linear combination of the prediction errors at the previous timestamps of length q, where q is the order of the moving average component
   
   \begin{equation}
       MA(q) =  \sum_{i=1}^{q} b_{i}.\epsilon_{t-i} + \mu + \epsilon_{t}
   \end{equation}
   
   where $b_{i}$ and q are the coefficients and the order of the MA model respectively. 
    
   The AR and MA component are enough to model a time series in the case the time series data is stationary i.e. the time series have the same values of certain properties(mean, variance) over every time interval. For non-stationary data the time series data is differenced to make the data stationary. 
   
   \begin{equation}
       Y_{t} = X_{t} - X_{t-r}
   \end{equation}
   
   where r is the order of differencing.
   
   The primary task in this type of modelling is estimating the coefficients $a_i$, $b_{i}$ of the AR, MA components of the model and the order p,q,r of the AR, MA and differencing respectively.  The Box and Jenkins \raha{reference} approach is used to estimate the parameters of an ARIMA model, assuming an  underlying  model,  and  verifying  if  the  residuals  or  error term is a random distribution.  This process is repeated with different models until the right model is obtained. The Simple Exponential Smoothing(SES) \cite{brown1956exponential} is a modification of the ARIMA model with exponential weights assigned to each observation. Double and Triple Exponential Smoothing(DES, TES) \cite{esm2002} handles non-stationary data by introducing an additional parameter $\beta$ for smoothing the trend in the series.  Additionally, a extra  parameter $\gamma$ is  introduced  in  TES  to  control  the influence of seasonality.
   
   
   
 %  RBM 
  
  The energy function, joint distribution between the hidden and visible nodes are given by :- 
    
    \begin{equation}
        E(x,h) = h^{T}Wx + b^{T}h + c^{T}v
        P(x,h) = \frac{1}{Z} \exp{E(x,h)}
    \end{equation}
    
    where Z is used to ensure a normalized distribution. 
    
    The probability of a hidden unit $h_{j}$ being activated given a visible vector x is given by - 
    
    \begin{equation}
        P(h_{j}|x) = \sigma(b_{j} + \sum_{i} W_{ij}x_{i})
    \end{equation}
    
    and the probability that a visible vector $x_{i}$ is activated given a hidden unit $h$ is given by - 
    
    
    \begin{equation}
        P(x_{i}|h) = \sigma(c_{i} + \sum_{j} W_{ij}h_{j})
    \end{equation}
    
    
    % Interval based features
    
       Features can also be extracted from the intervals of each series referred to as interval based features in time series literature. The dimensions of the feature space increases in this approach and methods are proposed to handle this huge dimensionality and effectively use this interval based features. Rodriguez et. al \cite{rodriguez2005} considers intervals with lengths of powers of two and calculates binary features using threshold rules on the mean and standard deviation of each interval. Deng et. al \cite{deng2013} uses the slope, standard deviation and mean of the intervals as features for a random forest whose evaluation points are pre-defined using a refined splitting criteria for choosing between equally valued information gain between features. This method is expanded in Baydogan et.al\cite{baydogan2013} by introducing various stages namely generating a subseries classification problem, forming class probability estimates of the subserieses, and then creating a bag of features of the series from these probabilities which is then used to create a random forest classifier. 
       
   % Generative vs Discriminative Models
   
   Generative models usually models the relationship between the variables at different timesteps P($x(1)$, $x(2)$,..., $x(t)$) by learning the joint distribution between the timesteps P($x(1)$, $x(2)$,..., $x(t)$)  whereas discriminative models try to model the conditional probability between the input time series and the output class variable given by P($Y|x(1)$, $x(2)$,..., $x(t)$). Broadly, the models can be end-to-end in the sense that the raw time-series data can be fed to the model and trained end-to-end, or there might be time-series specific feature extraction which converts the raw time-series into some feature space and various classifiers are used on this feature space. 
   
   
   % Types of classifiers
   
   There are three broad approaches for using discriminative models with time series data - using distance based classifiers such as kNN or SVM using distance measures specific to time series data, finding discriminative features from the time series data and using it as input for classifiers and deep learning based model which learns relevant discriminative features from the time series data in an unsupervised manner.
   
   % Applicatios of ESN
   
   Borovykh et. al\cite{Borovykh2017ConditionalTS} used WaveNet to forecast time series by approximating the joint distribution of the time series. The  forecasting  algorithm  can be extended to anomaly detection using a similar threshold based prediction error method.
   
   
    Munir et. al\cite{munir2018} uses a CNN with multiple convolution and max-pooling layers followed by a dense layer to predict the output at next time steps based on the size of the output. To detect anomalies similar method of prediction error comparison with threshold value is used. To reduce the vanishing gradient problem of CNN's residual networks were proposed in Wang et. al\cite{wang2017time}, but could overfit if the amount of data is small.

==> TimeSeriesModelling/timeSeriesModelingOld.tex <==
\section{Modeling Time series data}
A time series data is a sequence of real-valued data with each data point related to a timestamp. Mathematically, a time series data is denoted as X = ({$x_{1}(t)$, $x_{2}(t)$,..., $x_{k}(t)$}) where t denotes the timestamp and k is the dimension of the real-valued variable at each time step. The structure of time series data is different from the i.i.d data in terms of high feature correlation and high dimensionality of data. Additionally, there is inherent measurement induced noise in the data. The underlying pattern recognition techniques can be classified as generative or discriminative based on the probability distribution it models.

\raha{please reorganize, in the new subsections make sure you cover all the concepts we need to know to understand section 3 and 4}
   \subsection{Discriminative Models}
   
   Discriminative models for Time Series tries to extract features from the data(X) that can distinguish different classes(Y). Mathematically,  given a time series X = ({$x_{1}(t)$, $x_{2}(t)$,..., $x_{k}(t)$}) it tries to model P($Y|X$). In some line of work it extracts feature set F = {$f_{1}$, $f_{2}$,...,$f_{m}$} from the raw time series data and models P($Y|F$) using models for non-sequence data. 
   
%    \newline
   
   \anchit{Distance Based Classifiers}
   
  K-nearest neighbour(knn), Support Vector Machine(SVM) or decision trees using distance measures specific to time series data has been proposed for time series classification, where the focus is on defining time series specific distance measures to be used with these classifiers. Some of the most commonly used distance measures used for time series dataset are the euclidean distance and the Dynamic Time Warping(DTW) distance.
   
   \begin{definition}
      Euclidean Distance - Given two time series $X_{1} = (x_{1}, ..., x_{t})$ and $X_{2} = (x^{'}_{1}, ..., x^{'}_{t})$, the euclidean distance between $X_{1}$ and $X_{2}$ is given by $\sum_{i=1}^{n} (x_{i} - x^{'}_{i})^{2} $
     
   \end{definition}
   
   \begin{definition} 
     Dynamic Time Warping \cite{berndtDTW1994} - Given two time series $X_{1} = (x_{1}, ..., x_{t})$ and $X_{2} = (x^{'}_{1}, ..., x^{'}_{t^{'}})$, to find the DTW distance, a matrix M of size t by $t^{'}$ is constructed which consists of the distance between a given time stamp value of $X_{1}$ with give time stamp of $X_{2}$. Thus, the ith row and jth column of matrix M represented by $m_{ij}$ consists of the distance between the points $t_{i}$ and $t^{'}_{j}$, denoting the alignment between $t_{i}$ and $t^{'}_{j}$. The distance between two points is typically chosen to be a euclidean distance. A contiguous set of matrix elements, denoted as the warping path W, where the kth element is $w_{k} = (t_{k}, t^{'}_{k})$ and the warping path W = $w_{1},w_{2},..., w_{k},..., w_{K} $, where max(m,n) $\leq$ K $<$ m + n -1. For a warping path to be valid the following constraints need to be satisfied:- ($t_{1}, t^{'}_{1}$) = 1; ($t_{K}, t^{'}_{K}$) = (m,n); $0 \leq t_{k+1} t_{k} \leq 1 $; and $0 \leq t^{'}_{k+1} t^{'}_{k} \leq 1 $. The DTW distance is the warping path, among exponentially possible warping paths that minimizes the total distance subject to the constraints mentioned above.
   
   \end{definition}
   The most common classifier in this regard is the 1-NN classifier with the DTW distance measures \cite{hui2008} .In Jeong et.al \cite{Jeong2011} based on the warping distance, weighted penalties are defined which reduces the warping horizons. Another similar distance measure is proposed where the transformation of one series to another series is defined using new operations move, split and merge  \cite{stefan2013}. The distance measured described before are based on first order differences. Other distance measures also include distances from the difference domain. Batista et. al \cite{batista2014} proposes a weighting method to take into account complexity differences in time series. Measure of complexity is chosen as the sum of squares of first difference. A weighted combination of the original time series and the first order differences are proposed in \cite{gorecki2013} referred as DDTW. DDTW combined with date transformed distances such as sin, cosine and Hilbert transform is proposed in \cite{gorecki2014}.
  
  \anchit{Word Representation Based Distance Measures}
  
   The time series dimensions is reduced by transforming them into word representations and similarity is measured based on the word distributions. The crux of this approach is to pass a window over the time series, approximating each window and then assigning symbols to the range of values thus creating discrete representations.
    Piecewise Aggregate Approximation(PAA) \cite{keogh2001dimensionality} reduces the raw time series dimensions by taking average value of fixed length intervals of the time series. For a time series X = ($x_{1}, x_{2}, ... , x_{m} $) with a dimension of m, the compressed time series $\hat{X}$ = ($\hat{x}_{1},\hat{x}_{2}, ..., \hat{x}_{n} )$ with a dimension n is obtained by :- 
      
      \begin{equation}
          \hat{x}_{k} = \frac{1}{e_{k} - s_{k} + 1} \sum_{i = s_{k}} ^{e_{k}} x_{i}
      \end{equation}
 
     Symbolic Aggregate Approximation(SAX) \cite{Lin2003},a method  to convert a numeric time series representation into a symbolic representation, builts upon the PAA framework by dividing the time series into equal segments, averaging, and  mapping every value to a string. To map the values to a string equiprobable regions are created from the distribution space, and each region is represented by a symbol. The PAA transformed time series $\hat{X}$ is converted to a string representation S = ($s_{1}, ...,s_{w}$).
     Lin et. al\cite{lin2012} applies Symbolic Aggregate Approximation (SAX) \cite{Lin2003} based on PAA \cite{keogh2001dimensionality} to the windows to get a word representation for each window. A count histogram is created over the word distribution of the time series and the euclidean distance between the count histograms are used as a distance measure for the 1-NN classifier. Instead of creating the word distributions over the time series, Senin et. al\cite{senin2013} creates word distributions over classes using tf-idf to weigh the distribution, using SAX representation and the vector space model in Information Retrieval. 
   
   \anchit{Feature Based Classifiers}
   The next set of models uses time-series specific features as inputs to discriminative classifiers. One of the features used extensively in time series models are shapelets, which are essentially subsequences of a time series that can discriminate among class memberships, and are representative of a class.
   \begin{definition}
    Shapelet. For a time series dataset X, consisting of two classes, $Y_{a}$ and $Y_{b}$,the subsequence shapelet(X) is such that, 
         Gain(shapelet(X), $d_{OSP(X,shapelet(X))}$) $\geq$ Gain(S, $d_{OSP(X,S)}$), where S is any other subsequence, $d_{OSP}$ is the optimal split point, and Gain refers to entropy based information gain. 
   \end{definition} 
   A shapelet splitting criteria based decision tree was proposed in Ye et. al\cite{yeKeogh2011}. An extension to the decision tree based approach was proposed in Rakthanmanon et. al\cite{rakthanmanon2013fast} to discover shapelets faster by discretising and approximating the shapelets instead of doing a full enumerative search. A dictionary of SAX words are formed for each possible shapelets, followed by random masking of letters and building frequency count histograms for each class. Based on how well the frequency histograms separate the classes the top k SAX words are chosen. Hills et. al\cite{hills2014}, Bostrom et. al\cite{Bostrom2015BinaryST} detach the shapelet discovery and the classifier by finding the top k shapelets in a single pass, and the shapelets are used to transform the dataset based on the distance between the series and a shapelet. Enumerative search for shapelets is replaced by a heuristic gradient descent shapelet search algorithm in Grabocka et. al\cite{grabocka2014}. 
   
   Using ensembles of different classifiers has worked really well for time series classification. Lines et. al\cite{lines2015} uses a ensemble of 1-NN classifiers with different distance measures and the cross-validation training accuracy is used as the voting scheme for the weights. Bagnall et. al \cite{bagnall2015} one of most successful classifiers in TSC uses a ensemble of classifiers in different domains such as time, shapelet, autocorrelation and power spectrum domain. 
   
   \anchit{Deep learning based classification methods}
   
   Deep learning based methods are proposed for Time Series Classification using hand crafted feature engineering approaches as well as end-to-end deep learning approaches. In the most basic form, a Deep Neural Network consisting of Multi Layer Perceptron(MLP) is used \cite{wang2016time}, which takes the raw time series as the input to 4 fully connected layers, with ReLU activations in the hidden layers and a softmax activation at the output layer. To prevent overfitting dropout operation is proposed at every layer. Fully Convolution Neural Networks(FCNNs) \cite{wang2016time} consists of convolutional layers without any local pooling layers thus keep the time series length constant across the convolutions. Additionally, the final FC layer is replaced by a Global Average Pooling(GAP) layer. The result of the final layer is averaged over the entire time dimension(the GAP layer) followed by a  softmax classifier . A residual network based architecture is also proposed in Wang et. al\cite{wang2016time} followed by a GAP layer, to reduce the vanishing gradient effect\cite{he2015}. An architecture similar to the FCNN architecture with the GAP layer replaced by an attention layer is proposed in Serra et. al\cite{serra2018}. The attention layer helps in learning the parts of the time series important for classification.  
   
   Different from the previous models Cui.et. al\cite{cui2016} doesn't take the raw time series as input and instead extract subsequences by passing a sliding window on the time series to train the network. The extracted subsequences are transformed with the following three mappings:- identity mapping, down-sampling and smoothing, resulting in an multivariate time series from an input univariate time series. The subsequences are passed to three convolution layers in parallel, and concatenated before passing to the subsequent convolution layers. Time Le-Net \cite{Guennec2016DataAF} inspired by LeNet architecture's success in document recognition consists of a traditional CNN with two convolutions, an FC layer followed by a softmax classifier. Zheng et.al\cite{zheng2014} proposes a deep CNN for multivariate time series data by applying the convolutions parallelly on each input channel of the MTS. Each time series channel go through two convolution layers with ReLU activation followed by a max pooling operation. After the second convolution layers the outputs of the two channels are concatenated and then passed to a FC layer followed by softmax classifier.
 
   Another popular architecture to model time series is the Echo State Network(ESN) \cite{Jaeger78}. ESN's were designed to reduce the vanishing gradient problem of the RNN's by removing the need to learn the weight's of the hidden layers. This also reduces the training time for the network which is beneficial for long time series sequences. The hidden layers in an ESN are randomly initialized and sparsely connected which is referred as the reservoir. Each neuron in the reservoir learns a non-linear representation of the input. The reservoir is followed by a fully connected output layer whose weights are learned by gradient descent. The internal hidden state activity at time t(I(t)) is calculated using the hidden state activity at t-1(I(t-1)) and the input element at time t(X(t)). 
   
   \begin{equation}
       I(t) = f(W_{in}X(t) + WI(t-1)), \forall t \in [1, T]
   \end{equation}
   
   where $W_{in}$ is the weight matrix for input time series, W is the internal connections of the reservoir. The output Y(t) is calculated using $Y(t) = W_{out}I(t)$.
  
   The effectiveness of ESN's depends highly on the initialization of the reservoir weights, which should follow the spectral radius property. Echo state networks(ESN) were used to reconstruct the time series in \cite{Aswolinskiy2017} \cite{bianchi2018} \cite{choukhi2018} \cite{ma2016} where the reservoir space was utilised to learn a representation of the series. Chen et. al,\cite{Chen2015ModelMC} Che et. al\cite{Che2017DECADEA} used a kernel over the learned representation over the ESN reservoir space followed by an SVM or MLP. Tanisaro et.al \cite{tanisaro2016} projected every timestamp of a timeseries to a higher dimension using the reservoir. A ridge classifier is used to predict the time series class.
   
    \subsection{Generative Models}
   
   Generative Models for time series analysis learn the joint probability distribution between the input time-dependent variables. A generative model for time series needs to learn  the distributions of features within each time point, P($x(1)$, $x(2)$,..., $x(t)$) along with the potentially complex dynamics of those variables. Specifically, we also need to capture $p(x_{t}|x_{1:t-1})$ across time.
   
   \anchit{State Space Models}
   
   State Space models, uses a latent state $l_{t} $ to model the time series data, encoding time series components level, trend and seasonality patterns. A SSM is denoted by a state-transition equation, which describes the transition dynamics $p(l_{t}|l_{t-1})$ of the evolution of the latent state over time, and an observation model which describes the conditional probability $p(x_{t}|l_{t})$ of observations given the latent state. Mathematically, an SSM is given by 
   
   \begin{equation}
       l_{t+1} = f(l_{t}, x_{t}) + \epsilon_{t},
       y_{t} = g(l_{t}, x_{t}) + \gamma_{t}
   \end{equation}
   

    For more complex, noisy and higher dimensional real world data model assumption techniques such as ARIMA is not an efficient technique since the dynamics are unknown or too complex \cite{Taylor2009ComposableDM}. Various unsupervised generative models have been extended for time series data to solve this problem. Graves et. al \cite{gravesRNN2013} proposed a method for sequence generation using recurrent models such as RNN and LSTM, by processing the real data at each step($x_{t}$) and predicting the value of the next step($x_{t+1}$). Output predictions($y_{t}$) at each step are made probabilistic, and is sampled from to be fed as the next step input. Iteratively sampling at each step from the already trained network, and passing to the next step produces a  novel sequence. Although, theoretically possible, RNNs in practice suffer to capture long term dependencies and thus LSTM's are used which are shown to capture long term dependencies with the help of various gating mechanisms. Additionally, the hidden layers are stacked to increase the depth across space to allow for higher non-linearities to be captured at each time step. The probability of the input sequence x is given by Pr(x) = $\prod_{t=1}^{T}Pr(x_{t+1}|y_{t})$. 
    
    In other work an extension for the Restricted Boltzmann Machine(RBM), a generative probabilistic model between the input nodes(visible) and latent nodes(hidden), connected by a weight matrix(W) and having associated bias vectors c and b respectively, which is trained by minimizing the reconstruction error using contrastive divergence\cite{Hinton2002a} is proposed. 
    
    Conditional RBM and temporal RBM \cite{SutskeverH07} extends the RBM model with connection between the current hidden units and the past visible units along with auto-regressive weights for capturing short-term temporal patterns. The dependency between the bias vectors and the past visible units are defined by - 
    
    \begin{equation}
        b_{j}^{'} = b_{j} + \sum_{i}^{n} B_{i} x(t-i),
        c_{i}^{'} = c_{i} + \sum_{i}^{n} A_{i} x(t-i)
    \end{equation}
    
    where $B_{i}$ and $A_{i}$ are the weight matrices connecting current hidden units to visible units at time t-i, and current visible units to visible units at time t-i respectively. Thus the conditional probabilities for activation of the hidden units and the visible units become:- 
    
    \begin{equation}
        P(h_{j}|x) = \sigma(b_{j} + \sum_{i} W_{ij}x_{i}) + \sum_{k}\sum_{i} B_{ijk} x_{i}(t-k)
    \end{equation}
    
    \begin{equation}
        P(x_{i}|h) = \sigma(c_{i} + \sum_{i} W_{ij}h_{j}) + \sum_{k}\sum_{i} A_{ijk} x_{i}(t-k)
    \end{equation}

   Oord et.al\cite{oord2016} proposed a CNN based architecture called Wavenet to generate audio waveforms.  The wavenet tries to approximate the joint probability of the time series $X = ({x_{1}, x_{2}, ..., x_{T}}$) by making x depend on all the previous samples. 
   WaveNet uses a special convolutional layer called the dilated causal convolution. A causal convolution forces the prediction at any timestep to depend on the previous timesteps and  prevents dependencies on future timesteps. Dilated convolutions is a filter which can span larger than it's length by dilation with zeros, skipping input values at some steps, thus increasing the receptive field of the filters with increasing depth. Additionally, gated activated units are used which allows the network the ability to preserve and forget certain input values. Other work in time series modelling includes Undecimated Fully Convolutional Network(UFCNN) \cite{mittelman2015} where Fully Convolutional Layers where 1-D causal filters are used, and the filter's at $l^{th}$ resolution level is upsampled by a factor of $2^{l-1}$ along the time dimension along with removal of max-pooling layers and other upsampling operators.
   
   \anchit{GAN based}
    Generative Adversarial Network(GAN) based models has also been proposed for Time Series Generation . Mogren et. al\cite{mogrenCRNN2016} proposed C-RNN-GAN to generate continuous sequential data by modelling the joint probability distribution of the sequence. The generator was designed using a LSTM and the discriminator consisted of a bidirectional RNN. The model was trained using the standard GAN loss. Yoon et.al\cite{yoonTSGAN2019} argued that using recurrent networks for the generator and discriminator, and summing the GAN loss over sequences is not enough for capturing the temporal dynamics of the data. They proposed introducing a stepwise supervised loss along with the unsupervised adversarial loss to encourage the model to capture the stepwise temporal dependencies. 
